Et Tu Certifications: Robustness Certificates Yield Better Adversarial Examples

In guaranteeing the absence of adversarial examples in an instance's neighbourhood, certification mechanisms play an important role in demonstrating neural net robustness. In this paper, we ask if these certifications can compromise the very models they help to protect? Our new \emph{Certification Aware Attack} exploits certifications to produce computationally efficient norm-minimising adversarial examples $74 \%$ more often than comparable attacks, while reducing the median perturbation norm by more than $10\%$. While these attacks can be used to assess the tightness of certification bounds, they also highlight that releasing certifications can paradoxically reduce security.

==> consolidated_tab.tex <==
\begin{table}
  \caption{Performance metrics for MNIST (M), Cifar-$10$ (C), and Tiny-Imagenet (TI) for varying $\sigma$. `Success' and `Best' are the proportion samples for which each attack was success, and outperformed all others. $r_{50}$ and $\%$-Cohen are the median attack and the size relative to the guarantee of Cohen. } %
  
  \label{tab:times}
  \centering
  \begin{tabular}{lllllllll}
    \toprule
    \multicolumn{2}{c}{Categorisation} & \multicolumn{5}{c}{Smallest Attack} & \multicolumn{2}{c}{First Attack}\\
Data & Attack & Success & Best & $r_{50}$ & $\%$-Cohen & Time (s) & Ratio$(r_{50})$ & Ratio$($Time$)$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
M-$0.5$ & 	 Ours & 	 $75\%$ & 	 $71\%$ & 	 $1.95$ & 	 $67\%$ & 	 $5.49$ & 	 $1.10$ & 	 $0.23$\\
 & 	 PGD & 	 $65\%$ & 	 $6\%$ & 	 $1.95$ & 	 $69\%$ & 	 $8.95$ & 	 $1.00$ & 	 $0.34$\\
 & 	 C-W & 	 $94\%$ & 	 $25\%$ & 	 $8.19$ & 	 $612\%$ & 	 $5.29$ & 	 $1.63$ & 	 $0.02$\\
 & 	 Auto & 	 $31\%$ & 	 $2\%$ & 	 $1.95$ & 	 $100\%$ & 	 $174.87$ & 	 $1.00$ & 	 $1.00$\\
 & 	 D.Fool & 	 $5\%$ & 	 $1\%$ & 	 $9.20$ & 	 $2107\%$ & 	 $0.66$ & 	 $1.00$ & 	 $1.00$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
M-$1.0$ & 	 Ours & 	 $100\%$ & 	 $89\%$ & 	 $2.41$ & 	 $66\%$ & 	 $2.87$ & 	 $1.09$ & 	 $0.43$\\
 & 	 PGD & 	 $98\%$ & 	 $4\%$ & 	 $2.75$ & 	 $88\%$ & 	 $8.92$ & 	 $1.00$ & 	 $0.43$\\
 & 	 C-W & 	 $94\%$ & 	 $0\%$ & 	 $8.83$ & 	 $505\%$ & 	 $4.49$ & 	 $1.51$ & 	 $0.03$\\
 & 	 Auto & 	 $90\%$ & 	 $6\%$ & 	 $3.05$ & 	 $100\%$ & 	 $174.08$ & 	 $1.00$ & 	 $1.00$\\
 & 	 D.Fool & 	 $47\%$ & 	 $0\%$ & 	 $12.80$ & 	 $1409\%$ & 	 $0.65$ & 	 $1.00$ & 	 $1.00$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
C-$0.5$ & 	 Ours & 	 $96\%$ & 	 $83\%$ & 	 $0.85$ & 	 $69\%$ & 	 $3.34$ & 	 $1.23$ & 	 $0.19$\\
 & 	 PGD & 	 $95\%$ & 	 $3\%$ & 	 $0.97$ & 	 $88\%$ & 	 $9.19$ & 	 $1.00$ & 	 $0.14$\\
 & 	 C-W & 	 $95\%$ & 	 $2\%$ & 	 $6.65$ & 	 $1104\%$ & 	 $4.58$ & 	 $2.07$ & 	 $0.03$\\
 & 	 Auto & 	 $85\%$ & 	 $11\%$ & 	 $1.27$ & 	 $100\%$ & 	 $179.28$ & 	 $1.00$ & 	 $1.00$\\
 & 	 D.Fool & 	 $90\%$ & 	 $0\%$ & 	 $2.39$ & 	 $512\%$ & 	 $0.67$ & 	 $1.00$ & 	 $1.00$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
C-$1.0$ & 	 Ours & 	 $100\%$ & 	 $85\%$ & 	 $1.24$ & 	 $79\%$ & 	 $2.38$ & 	 $1.13$ & 	 $0.38$\\
 & 	 PGD & 	 $100\%$ & 	 $1\%$ & 	 $1.55$ & 	 $114\%$ & 	 $9.17$ & 	 $1.00$ & 	 $0.22$\\
 & 	 C-W & 	 $95\%$ & 	 $0\%$ & 	 $6.76$ & 	 $775\%$ & 	 $4.43$ & 	 $2.01$ & 	 $0.03$\\
 & 	 Auto & 	 $74\%$ & 	 $12\%$ & 	 $1.88$ & 	 $100\%$ & 	 $178.91$ & 	 $1.00$ & 	 $1.00$\\
 & 	 D.Fool & 	 $98\%$ & 	 $1\%$ & 	 $3.05$ & 	 $462\%$ & 	 $0.67$ & 	 $1.00$ & 	 $1.00$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
T-I-$0.5$ & 	 Ours & 	 $94\%$ & 	 $77\%$ & 	 $0.97$ & 	 $89\%$ & 	 $6.62$ & 	 $1.18$ & 	 $0.23$\\
 & 	 PGD & 	 $93\%$ & 	 $1\%$ & 	 $1.15$ & 	 $113\%$ & 	 $18.80$ & 	 $1.00$ & 	 $0.17$\\
 & 	 C-W & 	 $100\%$ & 	 $6\%$ & 	 $11.79$ & 	 $1981\%$ & 	 $13.76$ & 	 $2.45$ & 	 $0.02$\\
 & 	 Auto & 	 $67\%$ & 	 $15\%$ & 	 $1.38$ & 	 $100\%$ & 	 $360.88$ & 	 $1.00$ & 	 $1.00$\\
 & 	 D.Fool & 	 $79\%$ & 	 $1\%$ & 	 $2.39$ & 	 $532\%$ & 	 $1.36$ & 	 $1.00$ & 	 $1.00$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
T-I-$1.0$ & 	 Ours & 	 $95\%$ & 	 $84\%$ & 	 $1.37$ & 	 $107\%$ & 	 $4.70$ & 	 $1.13$ & 	 $0.44$\\
 & 	 PGD & 	 $94\%$ & 	 $1\%$ & 	 $1.80$ & 	 $161\%$ & 	 $19.51$ & 	 $1.00$ & 	 $0.26$\\
 & 	 C-W & 	 $100\%$ & 	 $5\%$ & 	 $10.73$ & 	 $1373\%$ & 	 $14.38$ & 	 $2.73$ & 	 $0.02$\\
 & 	 Auto & 	 $54\%$ & 	 $11\%$ & 	 $2.29$ & 	 $100\%$ & 	 $372.23$ & 	 $1.00$ & 	 $1.00$\\
 & 	 D.Fool & 	 $89\%$ & 	 $0\%$ & 	 $3.44$ & 	 $577\%$ & 	 $2.72$ & 	 $1.00$ & 	 $1.00$\\
    \bottomrule
  \end{tabular}
\end{table}


==> cutoff_tab.tex <==
\begin{table}
\centering
\caption{
Comparison of the influence of the cutoff $c$ in Our attack process for $\sigma = 0.5$, in terms of the median first and best adversarial example, and the median time for identifying the first adversarial example. 
} %
\label{tab:cutoff_metrics}
\begin{tabular}{@{}lccccc@{}}
\toprule
Dataset &  Cutoff $c$ & Successful & First $r_{50}$ & Best $r_{50}$ & First $t_{50}$ (s)  \\
\cmidrule(r){1-2} \cmidrule(r){3-6}
MNIST & $0.05$ & $45.0\%$ & $1.646$ & $1.617$ & $4.44$ \\
       & $0.25$ & $65.0 \%$ & $1.988$ & $1.874$ & $1.51$ \\ 
       & $0.5$ & $71.5 \%$ & $2.149$ & $1.942$ & $1.16$ \\
       & $0.75$ & $75.0 \%$ & $2.345$ & $1.962$ & $1.07$ \\ 
       &$1.0$ & $75.5 \%$ & $2.426$ & $1.972$ & $1.07$ \\
       & $1.5$ & $74.5 \%$ & $2.687$ & $1.993$ &  $0.97$ \\ 
       & $3.0$ & $74.0 \%$ & $3.257$ & $2.020$ & $0.97$ \\
\cmidrule(r){1-2} \cmidrule(r){3-6}
CIFAR-$10$ & $0.05$ & $93.5\%$ & $0.806$ & $0.756$ & $1.76$ \\
       & $0.25$ & $97.5 \%$ & $0.904$ & $0.801$ & $0.74$ \\ 
       & $0.5$ & $97.0 \%$ & $1.030$ & $0.807$ & $0.65$ \\
       & $0.75$ & $97.0 \%$ & $1.135$ & $0.814$ & $0.65$ \\ 
       &$1.0$ & $99.0 \%$ & $1.220$ & $0.838$ & $0.65$ \\
       & $1.5$ & $98.5 \%$ & $1.486$ & $0.829$ & $0.65$ \\ 
       & $3.0$ & $99.0 \%$ & $2.194$ & $0.845$ & $0.65$ \\
\bottomrule
\end{tabular}
\end{table}

==> first_metrics_tab.tex <==
\begin{table}
\centering
\caption{
Performance metrics for the \textit{first identified adversarial example} for MNIST (M), CIFAR-$10$ (C-$10$), and Tiny-Imagenet (T-I), based upon $250$ samples. Metrics include the median adversarial example, average time, and the ratio of these quantities to their respective variants in Table~\ref{tab:metrics}. %
}


\label{tab:metrics_first}
\resizebox{\linewidth}{!}{ %
\begin{tabular}{@{}lcc|cc|cc@{}}
\toprule
 Data   & $\sigma$ & Attack & $r_{50}$ & Ratio ($r_{50}$) & Time (s) & Ratio (Time) \\
\midrule
M & $0.5$ & Ours & $2.15$ & $1.12$ & $2.43$ & $0.29$\\
 &  & C-W & $13.35$ & $1.64$ & $0.18$ & $0.02$\\
\midrule
M & $1.0$ & Ours & $2.59$ & $1.08$ & $1.66$ & $0.37$\\
 &  & C-W & $13.35$ & $1.51$ & $0.18$ & $0.03$\\
\midrule
C-$10$ & $0.5$ & Ours & $1.02$ & $1.28$ & $1.04$ & $0.15$\\
 &  & C-W & $13.68$ & $2.09$ & $0.23$ & $0.03$\\
\midrule
C-$10$ & $1.0$ & Ours & $1.25$ & $1.15$ & $1.16$ & $0.28$ \\
 &  & C-W & $13.61$ & $2.13$ & $0.25$ & $0.03$ \\
 \midrule
T-I & $0.5$ & Ours & $1.09$ & $1.18$ & $1.33$ & $0.22$\\
 &  & C-W & $27.79$ & $2.61$ & $0.22$ & $0.02$\\
 \midrule
T-I & $1.0$ & Ours & $1.31$ & $1.14$ & $1.69$ & $0.42$\\
 &  & C-W & $29.21$ & $3.16$ & $0.22$ & $0.01$\\
\bottomrule
\end{tabular}
} %
\end{table}


==> macer-tab.tex <==
\begin{table}
  \caption{Performance metrics for MNIST (M), Cifar-$10$ (C), and Tiny-Imagenet (TI) for varying $\sigma$. `Success' and `Best' are the proportion samples for which each attack was success, and outperformed all others. $r_{50}$ and $\%$-Cohen are the median attack and the size relative to the guarantee of Cohen. } %
  
  \label{tab:macer_times}
  \centering
  \begin{tabular}{lllllllll}
    \toprule
    \multicolumn{2}{c}{Categorisation} & \multicolumn{5}{c}{Smallest Attack} & \multicolumn{2}{c}{First Attack}\\
Data & Attack & Success & Best & $r_{50}$ & $\%$-Cohen & Time (s) & Ratio$(r_{50})$ & Ratio$($Time$)$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
C-$0.25$ & 	 Ours & 	 $100\%$ & 	 $100\%$ & 	 $0.91$ & 	 $1188\%$ & 	 $17.54$ & 	 $1.20$ & 	 $0.35$\\
 & 	 PGD & 	 $100\%$ & 	 $0\%$ & 	 $15.17$ & 	 $20977\%$ & 	 $26.25$ & 	 $1.00$ & 	 $0.02$\\
 & 	 C-W & 	 $96\%$ & 	 $0\%$ & 	 $10.61$ & 	 $13958\%$ & 	 $4.04$ & 	 $1.30$ & 	 $0.08$\\
 & 	 D.Fool & 	 $100\%$ & 	 $0\%$ & 	 $2.10$ & 	 $3105\%$ & 	 $9.59$ & 	 $1.00$ & 	 $1.00$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
C-$0.5$ & 	 Ours & 	 $92\%$ & 	 $92\%$ & 	 $1.56$ & 	 $1148\%$ & 	 $19.33$ & 	 $1.08$ & 	 $0.55$\\
 & 	 PGD & 	 $100\%$ & 	 $0\%$ & 	 $15.58$ & 	 $11912\%$ & 	 $26.32$ & 	 $1.00$ & 	 $0.02$\\
 & 	 C-W & 	 $87\%$ & 	 $2\%$ & 	 $11.58$ & 	 $7242\%$ & 	 $3.37$ & 	 $1.23$ & 	 $0.10$\\
 & 	 D.Fool & 	 $100\%$ & 	 $5\%$ & 	 $4.28$ & 	 $3353\%$ & 	 $11.51$ & 	 $1.00$ & 	 $1.00$\\
\cmidrule(r){1-2} \cmidrule(r){3-7} \cmidrule(r){8-9}
C-$1.0$ & 	 Ours & 	 $75\%$ & 	 $75\%$ & 	 $2.03$ & 	 $1209\%$ & 	 $19.57$ & 	 $1.05$ & 	 $0.66$\\
 & 	 PGD & 	 $100\%$ & 	 $1\%$ & 	 $16.14$ & 	 $8101\%$ & 	 $26.24$ & 	 $1.00$ & 	 $0.02$\\
 & 	 C-W & 	 $99\%$ & 	 $11\%$ & 	 $11.29$ & 	 $5932\%$ & 	 $3.36$ & 	 $1.24$ & 	 $0.10$\\
 & 	 D.Fool & 	 $100\%$ & 	 $13\%$ & 	 $7.49$ & 	 $3984\%$ & 	 $9.61$ & 	 $1.00$ & 	 $1.00$\\
    \bottomrule
  \end{tabular}
\end{table}


==> new_consolidated_tab.tex <==
\begin{table}
  \caption{Performance metrics for Blah} %
  
  \label{tab:times_new}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    \multicolumn{3}{c}{Categorisation} & \multicolumn{4}{c}{Smallest Attack} \\
Dataset & $\sigma$ & Attack & Best & Success & Median $r$ & Median Time (s) \\
\cmidrule(r){1-3} \cmidrule(r){4-7}
mnist 	 & 	 $0.25$ 	 & 	 Ours 	 & 	 $9.16 \%$ 	 & 	 $12.75 \%$ 	 & 	 $1.02$ 	 & 	 $0.19$ \\
 	 & 	  	 & 	 PGD 	 & 	 $3.98 \%$ 	 & 	 $12.35 \%$ 	 & 	 $1.04$ 	 & 	 $2.52$ \\
 	 & 	  	 & 	 CW 	 & 	 $82.07 \%$ 	 & 	 $93.23 \%$ 	 & 	 $8.41$ 	 & 	 $1.49$ \\
 	 & 	  	 & 	 DeepF 	 & 	 $0.00 \%$ 	 & 	 $1.20 \%$ 	 & 	 $3.14$ 	 & 	 $0.17$ \\
\cmidrule(r){1-3} \cmidrule(r){4-7}   
& 	 $0.5$ 	 & 	 Ours 	 & 	 $35.86 \%$ 	 & 	 $72.91 \%$ 	 & 	 $2.02$ 	 & 	 $0.23$ \\
 	 & 	  	 & 	 PGD 	 & 	 $38.25 \%$ 	 & 	 $65.74 \%$ 	 & 	 $1.93$ 	 & 	 $2.66$ \\
 	 & 	  	 & 	 CW 	 & 	 $25.50 \%$ 	 & 	 $93.23 \%$ 	 & 	 $8.66$ 	 & 	 $1.50$ \\
 	 & 	  	 & 	 DeepF 	 & 	 $0.00 \%$ 	 & 	 $3.98 \%$ 	 & 	 $9.26$ 	 & 	 $0.17$ \\
\cmidrule(r){1-3} \cmidrule(r){4-7}
mnist 	 & 	 1.0 	 & 	 Ours 	 & 	 $72.11 \%$ 	 & 	 $100.00 \%$ 	 & 	 $2.64$ 	 & 	 $0.24$ \\
 	 & 	  	 & 	 PGD 	 & 	 $27.49 \%$ 	 & 	 $98.80 \%$ 	 & 	 $2.76$ 	 & 	 $2.56$ \\
 	 & 	  	 & 	 CW 	 & 	 $0.00 \%$ 	 & 	 $93.23 \%$ 	 & 	 $9.52$ 	 & 	 $1.11$ \\
 	 & 	  	 & 	 DeepF 	 & 	 $0.40 \%$ 	 & 	 $43.03 \%$ 	 & 	 $14.25$ 	 & 	 $0.17$ \\
\cmidrule(r){1-3} \cmidrule(r){4-7}
cifar10 	 & 	 0.25 	 & 	 Ours 	 & 	 $66.93 \%$ 	 & 	 $83.67 \%$ 	 & 	 $0.63$ 	 & 	 $0.11$ \\
 	 & 	  	 & 	 PGD 	 & 	 $15.54 \%$ 	 & 	 $84.06 \%$ 	 & 	 $0.69$ 	 & 	 $2.58$ \\
 	 & 	  	 & 	 CW 	 & 	 $15.14 \%$ 	 & 	 $94.82 \%$ 	 & 	 $7.45$ 	 & 	 $1.01$ \\
 	 & 	  	 & 	 DeepF 	 & 	 $0.80 \%$ 	 & 	 $71.31 \%$ 	 & 	 $2.30$ 	 & 	 $0.16$ \\
\cmidrule(r){1-3} \cmidrule(r){4-7}
cifar10 	 & 	 0.5 	 & 	 Ours 	 & 	 $74.50 \%$ 	 & 	 $94.02 \%$ 	 & 	 $0.92$ 	 & 	 $0.14$ \\
 	 & 	  	 & 	 PGD 	 & 	 $19.52 \%$ 	 & 	 $92.43 \%$ 	 & 	 $1.03$ 	 & 	 $2.64$ \\
 	 & 	  	 & 	 CW 	 & 	 $3.19 \%$ 	 & 	 $90.44 \%$ 	 & 	 $6.66$ 	 & 	 $1.37$ \\
 	 & 	  	 & 	 DeepF 	 & 	 $0.00 \%$ 	 & 	 $84.86 \%$ 	 & 	 $2.74$ 	 & 	 $0.17$ \\
\cmidrule(r){1-3} \cmidrule(r){4-7}
cifar10 	 & 	 1.0 	 & 	 Ours 	 & 	 $86.85 \%$ 	 & 	 $100.00 \%$ 	 & 	 $1.26$ 	 & 	 $0.19$ \\
 	 & 	  	 & 	 PGD 	 & 	 $10.36 \%$ 	 & 	 $100.00 \%$ 	 & 	 $1.48$ 	 & 	 $2.59$ \\
 	 & 	  	 & 	 CW 	 & 	 $0.00 \%$ 	 & 	 $95.62 \%$ 	 & 	 $7.03$ 	 & 	 $1.20$ \\
 	 & 	  	 & 	 DeepF 	 & 	 $1.99 \%$ 	 & 	 $98.41 \%$ 	 & 	 $3.25$ 	 & 	 $0.16$ \\
    \bottomrule
  \end{tabular}
\end{table}

==> performance_tab.tex <==
\begin{table}
\centering
\caption{
Proportion of attacked samples (Attacked) and best performing attack (Prob B), median radii and average time, with the best metrics bolded. Testing performed against MNIST (M), CIFAR-$10$ (C-$10$), and Tiny-Imagenet (T-I) across $250$ samples.
}


\label{tab:metrics}
\resizebox{0.93\linewidth}{!}{ %
\begin{tabular}{@{}lcc|cccc@{}}
\toprule
Data   & $\sigma$ & Attack & Attacked & Prop B & $r_{50}$ & Time (s) \\
\midrule
M & $0.5$ & Ours & $76.0\%$ & $\mathbf{68.8}\%$ & $\mathbf{1.92}$ & $8.4$ \\
 &  & PGD & $70.8\%$ & $8.0\%$ & $2.00$ & $4.9$ \\
 &  & DeepFool & $4.8\%$ & $0.0\%$ & $5.00$ & $\mathbf{1.2}$ \\
 &  & C-W & $\mathbf{94.4}\%$ & $22.4 \%$ & $8.14$ & $8.2$ \\
\midrule    
M & $1.0$ & Ours & $\mathbf{100}\%$ & $\mathbf{96.8}\%$ & $\mathbf{2.41}$ & $4.5$\\
 &  & PGD & $98.8\%$ & $2.8\%$ & $2.67$ & $5.2$\\
 &  & DeepFool & $33.2\%$ & $0.4\%$ & $10.29$ & $\mathbf{1.0}$\\
 &  & C-W & $94.4\%$ & $0.0 \%$ & $8.84$ & $6.6$\\
\midrule
C-$10$ & $0.5$ & Ours & $\mathbf{97.6}\%$ & $\mathbf{94.4}\%$ & $\mathbf{0.80}$ & $6.9$\\
 &  & PGD & $96.0\%$ & $2.4\%$ & $0.91$ & $2.1$\\
 &  & DeepFool & $84.8\%$ & $3.2\%$ & $1.98$ & $\mathbf{1.2}$\\
 &  & C-W & $95.6\%$ & $2.0 \%$ & $6.54$ & $7.6$\\
\midrule
C-$10$ & $1.0$ & Ours & $\mathbf{100}\%$ & $\mathbf{97.2}\%$ & $\mathbf{1.09}$ & $4.1$\\
 &  & PGD & $\mathbf{100}\%$ & $0.8\%$ & $1.29$ & $2.8$\\
 &  & DeepFool & $92.8\%$ & $4.0\%$ & $2.67$ & $\mathbf{1.2}$\\
 &  & C-W & $95.2\%$ & $0.0 \%$ & $6.39$ & $8.1$\\
 \midrule
T-I & $0.5$ & Ours & $92.4\%$ & $\mathbf{88.4}\%$ & $\mathbf{0.92}$ & $6.1$\\
 &  & PGD & $91.6\%$ & $0.8\%$ & $1.12$ & $2.9$\\
 &  & DeepFool & $78.0\%$ & $8.4\%$ & $2.02$ & $\mathbf{1.5}$\\
 &  & C-W & $\mathbf{93.2}\%$ & $4.8 \%$ & $10.64$ & $13.3$\\
 \midrule
T-I & $1.0$ & Ours & $\mathbf{96.8}\%$ & $\mathbf{90.8}\%$ & $\mathbf{1.14}$ & $4.0$\\
 &  & PGD & $96.0\%$ & $2.0\%$ & $1.41$ & $4.0$\\
 &  & DeepFool & $88.0\%$ & $8.8\%$ & $2.49$ & $\mathbf{1.8}$\\
 &  & C-W & $\mathbf{96.8}\%$ & $2.8 \%$ & $9.25$ & $15.7$\\
\bottomrule
\end{tabular}
} %

\end{table}

%

%



